Exploring Strategies for Generalizable Commonsense Reasoning with Pre-trained Models

Commonsense reasoning benchmarks have been largely solved by fine-tuning language models. The downside is that fine-tuning may cause models to overfit to task-specific data and thereby forget their knowledge gained during pre-training. Recent works only propose lightweight model updates as models may already possess useful knowledge from past experience, but a challenge remains in understanding what parts and to what extent models should be refined for a given task. In this paper, we investigate what models learn from commonsense reasoning datasets. We measure the impact of three different adaptation methods on the generalization and accuracy of models. Our experiments with two models show that fine-tuning performs best, by learning both the content and the structure of the task, but suffers from overfitting and limited generalization to novel answers. We observe that alternative adaptation methods like prefix-tuning have comparable accuracy, but generalize better to unseen answers and are more robust to adversarial splits.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

% The task of commonsense reasoning has become very popular recently \cite{ma-etal-2019-towards, mitra2019exploring, shwartz-etal-2020-unsupervised, Bosselut2019DynamicKG, bauer-bansal-2021-identify}, while many of existing commonsense reasoning datasets are discriminative in nature \cite{talmor-etal-2019-commonsenseqa, sap-etal-2019-social, Bisk2020}, there have been numerous efforts for building generative benchmarks as well \cite{bhagavatula2019abductive, lin-etal-2020-commongen, boratko-etal-2020-protoqa}.

%The traditional task of 
Machine common sense reasoning has recently gained new traction, largely due to a novel set of diverse benchmarks~\cite{talmor-etal-2019-commonsenseqa, bhagavatula2019abductive, sap-etal-2019-social}, and the successful application of language modeling methods on these benchmarks~\cite{ma-etal-2019-towards, shwartz-etal-2020-unsupervised, bauer-bansal-2021-identify}.
The most widely adopted approach to solve these commonsense reasoning tasks is by fine-tuning large pre-trained language models (LMs)~\cite{devlin-etal-2019-bert, Liu2019RoBERTaAR} on the task-specific training data. Meanwhile, it has been shown that language models have acquired certain commonsense knowledge during their pre-training on large textual data~\cite{petroni2019language, davison-etal-2019-commonsense, ma2020knowledgedriven}. In light of these findings and the large capacity of the pre-trained language models, recent work has proposed lightweight alternatives to fine-tuning, by only updating a small amount of additional parameters~\cite{lin-etal-2020-exploring, li2021prefixtuning}, or updating the inputs while keeping the model weights intact~\cite{jiang-etal-2020-know, autoprompt:emnlp20}. Intuitively, these lightweight methods may retain the model's pre-trained knowledge to a large extent, and elicit the suitable knowledge for the target task, provided that much of this knowledge has already been encoded in the model parameters. However, to our knowledge, no comprehensive comparison exists between these model updating strategies. 

In this paper, we pose the question: \textit{What do models learn from commonsense reasoning datasets?} We consider three representative learning methods: regular fine-tuning, model extension with prefix-tuning \cite{li2021prefixtuning}, and model prompting with Autoprompt \cite{autoprompt:emnlp20}. We apply them to two model classes: the auto-regressive language model GPT-2 \cite{radford2019language} and sequence-to-sequence language model BART \cite{lewis-etal-2020-bart}. We conduct thorough evaluation on the generative evaluation benchmarks ProtoQA~\cite{boratko-etal-2020-protoqa} and CommonGen \cite{lin-etal-2020-commongen}, by training on different partitions of the training data. Our experiments show that fine-tuning performs best, by learning both the content and the structure of the task, but suffers from overfitting and limited generalization to novel answers. Prompting methods have lower accuracy, but tend to \cut{generalize better to unseen answers and to} show higher robustness to ``adversarial'' split. Extending the models by prefix-tuning represents a ``sweet spot'' between task accuracy, generalization, and robustness. 

% We consider two representative models and three families of learning methods. Our experiments show that fine-tuning performs best, by learning both the content and the structure of the task, but suffers from overfitting and limited generalization to novel answers. Prompting methods have lower accuracy, but tend to generalize better to unseen answers and to show higher robustness to adversarial examples. Extending the models by prefix-tuning represents a `sweet spot' between task accuracy, generalization, and robustness.


% we bridge this gap by experimenting with 3 different methods to train models to solve generative commonsense question answering tasks. We aim to provide evidences to shed light on the question "what has the model learned from each of these methods?". Specifically, we trained the auto-regressive language model GPT-2 \cite{radford2019language} and sequenece-to-sequence language model BART \cite{lewis-etal-2020-bart}, with fine-tuning, prefix-tuning \cite{li2021prefixtuning} and Autoprompt \cite{autoprompt:emnlp20}. We conducted thorough evaluation of our models on the recently introduced benchmark ProtoQA \cite{boratko-etal-2020-protoqa}, by training on different partitions of the training data. Our results suggests that fine-tuning mostly teaches the model to rely on lexical similarity matches to produce the answer predictions, without performing intended reasoning. Autoprompt on the other hands, has only learned the task structure, which makes it more robust towards an "adversarial" training split. 


%%% OLD INTRO %%%

% \section{Introduction}
% The task of commonsense reasoning has become very popular recently \cite{ma-etal-2019-towards, mitra2019exploring, shwartz-etal-2020-unsupervised, Bosselut2019DynamicKG, bauer-bansal-2021-identify}, while many of existing commonsense reasoning datasets are discriminative in nature \cite{talmor-etal-2019-commonsenseqa, sap-etal-2019-social, Bisk2020}, there have been numerous efforts for building generative benchmarks as well \cite{bhagavatula2019abductive, lin-etal-2020-commongen, boratko-etal-2020-protoqa}. The most widely adopted approach to solve these commonsense reasoning tasks is fine-tuning the pre-trained language models on the tasks' training data \cite{devlin-etal-2019-bert, radford2019language, Liu2019RoBERTaAR}, although it has been shown that language models have acquired a decent amount of commonsense knowledge from pre-training on large amount of unstructured text \cite{petroni2019language, davison-etal-2019-commonsense, tamborrino-etal-2020-pre, ma2020knowledgedriven}. Due to the large capacity of the pre-trained language models, another line of work has explored different alternatives to fine-tuning, i.e. lightweight tuning by only updating a small amount of additional parameters \cite{lin-etal-2020-exploring, li2021prefixtuning} or updating the inputs and keeping the model weights unchanged \cite{autoprompt:emnlp20}. Intuitively, these lightweight methods can retain the model's pre-trained knowledge to a large extent, and elicit the suitable knowledge for the target task. Thus, it's natural to apply these methods to commonsense reasoning tasks since the models has already encoded a good amount of commonsense knowledge in its parameters. However, to our knowledge, no prior work has experiments on this direction.\\
% In this paper, we bridge this gap by experimenting with 3 different methods to train models to solve generative commonsense question answering tasks. We aim to provide evidences to shed light on the question "what has the model learned from each of these methods?". Specifically, we trained the auto-regressive language model GPT-2 \cite{radford2019language} and sequence-to-sequence language model BART \cite{lewis-etal-2020-bart}, with fine-tuning, prefix-tuning \cite{li2021prefixtuning} and Autoprompt \cite{autoprompt:emnlp20}. We conducted thorough evaluation of our models on the recently introduced benchmark ProtoQA \cite{boratko-etal-2020-protoqa}, by training on different partitions of the training data. Our results suggests that fine-tuning mostly teaches the model to rely on lexical similarity matches to produce the answer predictions, without performing intended reasoning. Autoprompt on the other hands, has only learned the task structure, which makes it more robust towards an "adversarial" training split. 
